Decomposable Families of Itemsets

The problem of selecting a small, yet high quality subset of patterns from a larger collection of itemsets has recently attracted lot of research. Here we discuss an approach to this problem using the notion of decomposable families of itemsets. Such itemset families define a probabilistic model for the data from which the original collection of itemsets has been derived from. Furthermore, they induce a special tree structure, called a junction tree, familiar from the theory of Markov Random Fields. The method has several advantages. The junction trees provide an intuitive representation of the mining results. From the computational point of view, the model provides leverage for problems that could be intractable using the entire collection of itemsets. We provide an efficient algorithm to build decomposable itemset families, and give an application example with frequency bound querying using the model. Empirical results show that our algorithm yields high quality results.

==> theory.tex <==
\section{Partitions of Items}
\subsection{Definition}
A \emph{partition} $\prt{C} = \enset{C_1}{C_M}$ of the set of attributes $A$ is
a collection of pair-wise disjoint sets of attributes covering $A$. In other
words, $\bigcup_{i = 1}^M C_i = A$ and $C_i \cap C_j = \emptyset$, for $i \neq
j$. We define the entropy of partition to be
\[
\ent{\prt{C}} = \sum_{i = 1}^M \ent{C_i}.
\]

Given a partition $\prt{C}$ and a binary vector $v$, we define the probability of $A = v$
to be 
\[
\prob{A = v; \prt{C}} = \prod_{i = 1}^M \prob{C_i = v_{C_i}}.
\]

The log-likelihood for the whole data is
\[
\begin{split}
\log \prob{D; \prt{C}} & = \sum_{t \in D} \log \prob{A = t; \prt{C}} \\
                       & = \abs{D} \sum_{t \in \set{0, 1}^K} \prob{A = t; \prt{C}} \log \prob{A = t; \prt{C}} \\
					   & = -\abs{D} \ent{\prt{C}}.
\end{split}
\]
\subsection{Properties}
\subsection{Solving Algorithm}

\section{Trees of Items}
In the previous section we studied the partitions of attributes. In this
section we will relax the condition of having disjoint sets. We allow the sets
to overlap to some degree.  In order to do that we use tools from the theory of
Markov Random Fields.

\subsection{Definition}

Let $\cover{F} = \enset{F_1}{F_M}$ be an antichain cover of the set of
attributes $A$, that is, each attribute is occurring in at least one $F_i$ and
no $F_i$ is a subset of $F_j$. Just like for partitions we can also define a
define a distribution related to $\cover{F}$. The distribution is derived using
Maximum Entropy and its full treatment is given in XXX. We will denote the
entropy of such a distribution by $\ent{\cover{F}}$. The downside of this
approach is that solving the distribution for arbitrary $\cover{F}$ is \pp-hard
problem~\cite{XXX}.  Hence we are going to pay attention only in certain covers
whose entropy we can compute efficiently.

In order to do that we define a graph $G$ of $M$ nodes where the $i$th node
$n_i$ corresponds to $F_i$. Nodes $n_i$ and $n_j$ are connected if $F_i$ and
$F_j$ have a common attribute. The graph $G$ is called the \emph{clique graph}.

For notational simplicity we will assume that the clique graph $G$ is
connected; the extension of the following analysis for the non-connected graphs
is trivial. We are interested in spanning trees of $G$ having a \emph{running
intersection property}. To define this property let $\tree{T}$ be a spanning
tree of $G$. Let $F_i$ and $F_j$ be two sets having a common attribute, say,
$a$.  These sets are connected (w.r.t $\tree{T}$) by a unique path. Assume that
$a$ occurs in every $F_k$ along the path from $F_i$ to $F_j$. If this
assumption holds for any $F_i$, $F_j$, and a common attribute $a$, then we say
that tree has a running intersection property. Such a tree is called
\emph{junction tree}.

The entropy of a junction tree $\tree{T}$ is
\[
\ent{\tree{T}} = \sum_{X \in \vrt{\tree{T}}} \ent{X} - \sum_{Y \in \sep{\tree{T}}} \ent{Y}.
\]

We should point out that the clique graph can have multiple junction trees and
that not all spanning trees are junction trees. In fact, it may be the case
that the clique graph does not have junction trees at all. If, however, the
clique graph has a junction tree, we call the original cover $\cover{F}$
\emph{decomposable}.

\begin{theorem}
The entropies of a decomposable cover $\cover{F}$ and its junction tree
$\tree{T}$ are equal, that is, $\ent{\tree{T}} = \ent{\cover{F}}$. Moreover, if
$\tree{U}$ is also a junction tree for $\cover{F}$, then $\ent{\tree{U}} =
\ent{\tree{T}}$.
\end{theorem}

We assign to each edge $\pr{F_i, F_j}$ of a given junction tree $\tree{T}$ a
set of mutual attributes $F_i \cap F_j$. This set is called \emph{separator}.
We denote the set of all separators by $\sep{\tree{T}}$. We also denote the set
$\cover{F}$ by $\vrt{\tree{T}}$.

Given a junction tree $\tree{T}$ and a binary vector $v$, we define the probability of $A = v$
to be 
\[
\prob{A = v; \tree{T}} =  \prod_{X \in \vrt{\tree{T}}} \prob{X = v_{X}} \Big/ \prod_{Y \in \sep{\tree{T}}} \prob{Y = v_{Y}}.
\]

The log-likelihood for the whole data is
\[
\begin{split}
\log \prob{D; \tree{T}} & = \sum_{t \in D} \log \prob{A = t; \tree{T}} \\
                        & = \abs{D} \sum_{t \in \set{0, 1}^K} \prob{A = t; \tree{T}} \log \prob{A = t; \tree{T}} \\
					    & = -\abs{D} \ent{\tree{T}}.
\end{split}
\]

\subsection{Properties}

Similar to partitions we can define a concept of refinement for the covers.
Given two antichain covers $\cover{F}$ and $\cover{G}$. We say that $\cover{F}$
refines $\cover{G}$, if for each $X \in \cover{F}$, there is a $Y \in
\cover{G}$ such that $X \subseteq Y$.

\begin{theorem}
If $\cover{F}$ is a refinement of $\cover{G}$, then $\ent{F} \geq \ent{G}$.
\end{theorem}

\subsection{Finding Trees with Low Entropy}
In this section we describe the algorithm for searching decomposable covers.
To be more precise, given a downward closed family $\cover{F}$ covering the
set of attributes $A$, our goal is to construct a junction tree $\tree{T}$
with low entropy such that $\vrt{\tree{T}} \subseteq \cover{F}$. The final
output will be $\closure{\vrt{\tree{T}}}$, that is, the cliques of $\tree{T}$
along with their subsets.


We search the tree in an iterative fashion. At the beginning of each iteration
round we have a junction tree $\tree{T}_{n - 1}$ whose cliques have at most $n$ attributes.
The first tree is $\tree{T}_0$ containing only single attributes and no edges.
During the round the tree is modified so that in the end we will have
$\tree{T}_n$, a tree with cliques having at most $n + 1$ attributes.

In order to fully describe the algorithm
we need the following definition: $X$ and $Y$ are said to be \emph{$n-1$-connected} 
in a junction tree $\tree{T}$, if there is a path in $\tree{T}$ from $X$ to $Y$
having at least one separator of size $n-1$. We say that $X$ and $Y$ are $0$-connected,
if $X$ and $Y$ are not connected.

Each round of the algorithm consists of three steps. The pseudo-code of the algorithm
is given in Algorithm~\ref{alg:searchtree}--\ref{alg:modifytree}.
\begin{enumerate}
\item \textbf{Generate:} We construct a graph $G_n$ whose nodes are the cliques
of size $n$ in $\tree{T}_{n - 1}$. The edges of $G_n$ have the form $\pr{X, Y}$ 
such that $\abs{X \cap Y} = n - 1$ and $X \cup Y \in \cover{F}$.
We also set $\tree{T}_n = \tree{T}_{n - 1}$. The weight of the edge is
set to
\[
w\pr{e} = \ent{X} + \ent{Y} - \ent{X \cap Y} - \ent{X \cup Y}.
\]
\item \textbf{Augment:} We select the edge, say $e = \pr{X, Y}$ having largest
weight and remove it from $G_n$. If $X$ and $Y$ are not connected or $n - 1$
connected in $\tree{T}_n$ we proceed by modifying $\tree{T}_n$:
The tree $\tree{T}_n$ is augmented with a clique $V = X \cup Y$. For each $v \in V$,
we consider $W = V - v$. If $W$ is not in $\tree{T}_n$, it is added into
$\tree{T}_n$. $W$ is also added into $G_n$ and possibly new edges are added using
the same criteria as in the first step. We also connect $W$ and $V$ in
$\tree{T}_n$. A possible cycle is removed from $\tree{T}_n$ by finding an edge
with separator of size $n - 1$. Augmenting is repeated as long as $G_n$ is not empty.

\item \textbf{Purge:} The set $\vrt{\tree{T}_n}$ is not antichain if augmentation
has been performed. We purge the tree by keeping only the maximal sets of $\tree{T}_n$.
\end{enumerate}

To illustrate the algorithm we provide a toy example.

\begin{example}
Consider that we have a cover 
\[
\cover{F} = \set{a, b, c, d, ab, ac, ad, bc, bd, cd, abc, acd, bcd}.
\]

Assume that we are at the beginninh the second round and we have already the junction tree $\tree{T}_1$
given in Figure~\ref{fig:searchtree_example:a}. We form $G_2$ by taking the edges $\pr{ab, bc}$ and
$\pr{bc, cd}$. 

Consider that we pick $ab$ and $bc$ for joining. This will spawn $ac$ and $abc$ in $\tree{T}_2$ (Figure~\ref{fig:searchtree_example:d})
and $ac$ in $G_2$ (Figure~\ref{fig:searchtree_example:e}). Note that we also add the edge $\pr{ac, cd}$ into $G_2$.
Assume that we continue by picking $\pr{ac, cd}$. This will spawn $acd$ and $cd$ into $\tree{T}_2$. Note
that $\pr{bc, cd}$ is removed from $\tree{T}_2$, since otherwise we would have a cycle.

The last edge $\pr{bc, cd}$ is not added into $\tree{T}_2$ since $bc$ and $cd$ are not $n-1$-connected.
The final tree (Figure~\ref{fig:searchtree_example:g}) is obtained by keeping only the maximal sets, that is, removing the
cliques $bc$, $ab$, $ac$, $ad$, and $cd$.

\begin{figure}[htb!]
\center
\subfigure[$\tree{T}_1$, $\tree{T}_2$ at the beginning.]
	{\label{fig:searchtree_example:a}\begin{minipage}[b]{4cm}\center\includegraphics[scale=0.4]{pics/tree_ex1pic1}\end{minipage}}
\subfigure[$G_2$ at the beginning.]
	{\label{fig:searchtree_example:c}\begin{minipage}[b]{4cm}\center\includegraphics[scale=0.4]{pics/tree_ex1pic3}\end{minipage}}
\subfigure[$\tree{T}_2$ after joining $ab$ and $bc$.]
	{\label{fig:searchtree_example:d}\includegraphics[scale=0.4]{pics/tree_ex1pic4}}
\subfigure[$G_2$ after joining $ab$ and $bc$.]
	{\label{fig:searchtree_example:e}\includegraphics[scale=0.4]{pics/tree_ex1pic5}}
\subfigure[$\tree{T}_2$ after joining $ac$ and $cd$.]
	{\label{fig:searchtree_example:f}\includegraphics[scale=0.4]{pics/tree_ex1pic6}}
\subfigure[Final $\tree{T}_2$]
	{\label{fig:searchtree_example:g}\includegraphics[scale=0.4]{pics/tree_ex1pic7}}
\caption{Example of graphs during different stages of \textsc{SearchTree} algorithm.}
\label{fig:searchtree_example}
\end{figure}


\end{example}


\begin{algorithm}[ht!]
\caption{\textsc{SearchTree} algorithm. The input is a downward closed cover
$\cover{F}$, the output is a junction tree $\tree{T}$ such that $\vrt{\tree{T}} \subseteq
\cover{F}$.}
\begin{algorithmic}
\STATE $\vrt{\tree{T}_0} \define \set{x; x \in A}$ \COMMENT{$\tree{T}_0$ contains the single items.}
\STATE $n \define 0$.

\REPEAT
\STATE $n \define n + 1$.
\STATE $\tree{T}_n \define \tree{T}_{n - 1}$.
\STATE $\vrt{G_n} \define \set{X \in \vrt{\tree{T}_n}; \abs{X} = n}$.
\STATE $\edge{G_n} \define \set{\pr{X, Y}; X, Y \in \vrt{G_n}, \abs{X \cap Y} = n - 1, X \cup Y \in \cover{F}}$.

\REPEAT
\STATE $e = \pr{X, Y} \define \arg\max_{x \in \edge{G_n}} w(x)$. \COMMENT{Find the edge with the largest weight.}
\STATE $\edge{G_n} \define \edge{G_n} - e$.

\IF{$X$ and $Y$ are $n-1$-connected in $\tree{T}_n$}
\STATE Call \textsc{ModifyTree}.
\ENDIF

\UNTIL{$\edge{G_n} = \emptyset$}
\STATE Delete marked nodes from $\tree{T}_n$, connect the incident nodes.
\UNTIL{$G_n$ is empty}
\STATE \textbf{return} $\tree{T}$
\end{algorithmic}
\label{alg:searchtree}
\end{algorithm}


\begin{algorithm}[ht!]
\caption{\textsc{ModifyTree} algorithm.}
\begin{algorithmic}
\STATE $V \define X \cup Y$.
\STATE $\vrt{\tree{T}_n} \define \vrt{\tree{T}_n} + V$.
\FOR{$v \in V$}
\STATE $W \define V - v$.
\STATE Mark $W$.
\IF{$W \notin \edge{G_n}$}

\STATE $\vrt{G_n} \define \vrt{G_n} + W$.
\STATE $\edge{G_n} \define \edge{G_n} + \set{\pr{W, Z}; Z \in \vrt{G_n}, \abs{X \cap Z} = n - 1, V \neq X \cup Z \in \cover{F}}$.
\STATE $\vrt{\tree{T}_n} \define \vrt{\tree{T}_n} + W$.

\ENDIF
\STATE $\edge{\tree{T}_n} \define \edge{\tree{T}_n} + \pr{V, W}$.
\ENDFOR
\STATE Remove the possible cycle in $T_n$ by removing an edge $\pr{U, V}$ connecting
$X$ and $Y$ and having $\abs{U \cap V} = n - 1$.

\end{algorithmic}
\label{alg:modifytree}
\end{algorithm}


\begin{theorem}
Let $\tree{T}$ be a junction tree with cliques of size $n + 1$ at maximum.
Let $X, Y \in \vrt{T}$ be cliques of size $n$ such that $\abs{X \cap Y} = n - 1$.
Let $V = X \cup Y$. Then the family $\vrt{\tree{T}} + V$ is decomposable if and only
if $X$ and $Y$ are $n-1$-connected in $\tree{T}$.
\label{thr:junctionlegal}
\end{theorem}

\begin{proof}
The theorem is trivial for the case $n = 1$. Hence we assume that $n > 1$.

Assume that $X$ and $Y$ are $n-1$-connected in $\tree{T}$, and let $P$ be the
path connecting $X$ and $Y$. If $\pr{X, Y} \notin P$ , then there exists
$f = \pr{Z, W} \in P$ such that $\abs{Z \cap W} = n - 1$. Since $\tree{T}$
is a junction tree, we must have $Z \cap W = X \cap Y$. Hence by removing $f$
and adding $\pr{X, Y}$ does not violate the running intersection property.
Thus we can assume that $\pr{X, Y} \in \edge{\tree{T}}$. Adding $V$ between
$X$ and $Y$ does not violate the running intersection property and hence
$\vrt{\tree{T}} + V$ remains decomposable.

To prove the other direction assume that $X$ and $Y$ are not $n-1$ connected.
This implies that the path $P$ from $X$ to $Y$ consists of $n + 1$ cliques with
$n$ separators. Assume that $\vrt{\tree{T}} + V$ is decomposable and hence
there is a juncion tree $\tree{U}$ having $\vrt{\tree{U}} = \vrt{\tree{T}} + V$.
We can modify $\tree{U}$ such that the edges of the path $P$ occur in $\tree{U}$.
Let $P_s$ be the first clique in $P$ and let $P_l$ be the last.
Note that $V \subset P_s \cup P_l$. Let $P_e$ be the first clique in $P$ along the
path from $V$ to $P_s$. Since $\abs{P_s \cap V} = n$, we must have $P_e \cap V = P_s \cap V$
The path from $V$ to $P_e$ must also go through $P_e$, hence we must have
$P_s \cap V = P_l \cap V$. This implies that either $V = P_s$ or $V = P_l$, which
is a contradiction. This completes the proof.
\end{proof}

\begin{theorem}
\textsc{ModifyTree} decreases the entropy of $\tree{T}_n$ by $w(e)$.
\end{theorem}

\begin{proof}
Assume that the edge $e = \pr{X, Y} \in \edge{\tree{T}_n}$. Let $\tree{T}'_n$
be the tree after adding $X \cup Y$.
The entropy of the original tree is
\[
\ent{\tree{T}_n} = \ent{X} + \ent{Y} - \ent{X \cap Y} + B,
\]
where $B$ is the impact of the rest nodes. The entropy of the new tree is
\[
\ent{\tree{T}'_n} = \ent{X \cup Y} + B.
\]
Hence we have $\ent{\tree{T}_n} - \ent{\tree{T}'_n} = w(e)$.
\end{proof}

\begin{theorem}
If all the members of $\cover{F}$ of size $n + 1$ are added in $G_n$ at the
beginning of the $n$th round, then $\tree{T}_{n+1}$ has the has the lowest
entropy among the covers refined by $\tree{T}_n$ and containing the sets of
size $n + 1$, at maximum.
\end{theorem}

\begin{proof}
It is easy to see that the cliques $X$ and $Y$ are $n-1$ -connected if and
only if they are not connected by the previous edges from $G_n$. Hence, the
algorithm reduces to Krus\-kal's algorithm in finding the optimal spanning
tree of $G_n$, thus returning the optimal spanning tree.

Let $\tree{U}$ be a junction tree refined by $\tree{T}_n$ and containing the
cliques of size $n + 1$, at maximum. The cliques of size $n + 1$ occur in $G_n$.
Let $H$ be the corresponding edges in $G_n$. To prove the theorem we need to
show that $H$ contains no cycles.

Assume othewise, and consider adding the edges in $H$, one at the time.
When the first cycle occurs, the corresponding family is not decomposable by
Theorem~\ref{thr:junctionlegal}. The argument in the proof of Theorem~\ref{thr:junctionlegal}
holds even if we keep adding cliques of size $n + 1$, hence the final family cannot
be decomposable. Thus $H$ cannot contain cycles.
\end{proof}

\begin{corollary}
The tree $\cover{T}_1$ is optimal among the covers using the sets of size $2$.
\end{corollary}

